ITSRN++: Stronger and Better Implicit Transformer Network for Continuous Screen Content Image Super-Resolution

Nowadays, online screen sharing and remote cooperation are becoming ubiquitous. However, the screen content may be downsampled and compressed during transmission, while it may be displayed on large screens or the users would zoom in for detail observation at the receiver side. Therefore, developing a strong and effective screen content image (SCI) super-resolution (SR) method is demanded. We observe that the weight-sharing upsampler (such as deconvolution or pixel shuffle) could be harmful to sharp and thin edges in SCIs, and the fixed scale upsampler makes it inflexible to fit screens with various sizes. To solve this problem, we propose an implicit transformer network for continuous SCI SR (termed as ITSRN++). Specifically, we propose a modulation based transformer as the upsampler, which modulates the pixel features in discrete space via a periodic nonlinear function to generate features for continuous pixels. To enhance the extracted features, we further propose an enhanced transformer as the feature extraction backbone, where convolution and attention branches are utilized parallelly. Besides, we construct a large scale SCI2K dataset to facilitate the research on SCI SR. Experimental results on nine datasets demonstrate that the proposed method achieves state-of-the-art performance for SCI SR (outperforming SwinIR by 0.74 dB for x3 SR) and also works well for natural image SR. Our codes and dataset will be released upon the acceptance of this work.

==> Figure/ablition_modulation.tex <==
\begin{figure}
	\centering
	\footnotesize
	\begin{tabular}{c}
		\centering
		\begin{adjustbox}{valign=c}
			\begin{tabular}{c}
				\includegraphics[width=0.45\textwidth]{Image/freq/Freq_compare.png}
			\end{tabular}
		\end{adjustbox}
	\end{tabular}
	\caption{
	\textbf{ Frequency comparisons for different modulations in our implicit transformer.} We visualize the frequency of outputs under different modulations. Compare with other modulator, "sin" catches more high-frequency.
	}
	\label{fig:ablition-modulation}
\end{figure}

==> Figure/results_arbi.tex <==
\begin{figure*}
	\centering
	\footnotesize
	\begin{tabular}{c}
		\centering
		\begin{adjustbox}{valign=c}
			\begin{tabular}{c}
				\includegraphics[width=0.95\textwidth]{Image/result/arbi/arbs.png}
				% \\[1ex]
				% (c) Progressive upsampling (ours)
			\end{tabular}
		\end{adjustbox}
	\end{tabular}
	\caption{
	\textbf{Visualization on non-integer scale to show the ability of our continuous super-resolution}
	}
	\label{fig:result_arbi}
\end{figure*}

==> Table/arch_all.tex <==
\begin{table}[h]
    \centering
    \caption{
		\textbf{Ablation on the proposed Dual-Branch Block}. The module \textit{"parallel"} is our proposed DBB, where conv-branch and attention-branch are in parallel. The variant \textit{"sequential"} means the two branches are stacked sequentially. \textit{"conv\ only"} means we only use the conv-branch in our DBB, and \textit{"attention\ only"} means we only adopt the attention-branch in DBB. All the results are evaluated on the SCID dataset for $\times4$ SR. 
}
    \vspace{-3mm}
    \label{tab:arch_all}
    \resizebox{0.96\textwidth}{!}
    {
    \begin{tabular}{l|ccccc}
    % \hline
        \toprule[1.5pt]
        \multirow{2}{*}{\makecell[c]{Structure}}& 
        \multirow{2}{*}{\makecell[c]{Number of \\ Blocks} }& 
        \multirow{2}{*}{\makecell[c]{Embedding \\ Dims} } & 
        \multirow{2}{*}{\makecell[c]{Number of \\ Heads}} & 
        \multirow{2}{*}{\makecell[c]{Attention \\ Ratios} } & 
        \multirow{2}{*}{\makecell[c]{MLP 
        \\ Ratios}} 
        &
    
        &  & & & &
         \\ 
         \hline

    Fear & 13.98 M & 320.87 G & 27.84 & 0.9149 \\
    % \hline
    \bottomrule[1.5pt]
    \end{tabular}
    }
    % \vspace{cm}
\end{table}


==> Table/matmul_comparsion.tex <==
\begin{table}
	\centering
	\small 
	\caption{Matmul product vs. Hadamard product in implicit transformer for $\times 4$ evaluation on \textsc{SCID} } 
	\label{tab:multiplication}

	\setlength\tabcolsep{3.4pt}
	\begin{tabular}{l|ccc|c|c}
	
		\toprule[1.5pt]
	
		\multirow{2}{*}{} &  \multirow{2}{*}{Params.} & \multirow{2}{*}{FLOPs} & Latency &  PSNR & SSIM \\ 
		&&&&& \\ \hline
		Matmul
        & 22.62M & 888.67G & 107.76 & 27.63 & 0.9134 \\
        \hline
		Hadamard
        & 13.98M & 460.26 G & 350.08 ms & 27.42 dB & 0.9114 \\

		\bottomrule[1.5pt]
	\end{tabular}
\vspace{-2mm}
\end{table}

==> Table/para_mac.tex <==
\begin{table}
	\centering
	\small 
	\caption{Comparison of the proposed ITSRN++ architecture with existing SR  models on SCID dataset for $\times 4$ evaluation} 
	\label{tab:para_mac}

	\setlength\tabcolsep{3.4pt}
	\resizebox{0.48\textwidth}{!}{
	\begin{tabular}{l|ccc|c}
	
% 		\toprule[1.5pt]
	    \hline
		\multirow{2}{*}{Model} &  \multirow{2}{*}{Params.(M)} & \multirow{2}{*}{FLOPs(G)} & Peak GPU  &  PSNR \\ 
		&&&Memory(M)&(dB) \\ 
% 		\midrule
        \hline
	
		EDSR~\cite{lim2017edsr} & 43.09  & 1651.47   & 5087  & 25.85 \\
		RDN~\cite{zhang2018RDN}& 22.27  & 745.11 & 3415  & 26.11 \\
		RCAN~\cite{zhang2018rcan}
		& 15.59 & 522.47 & 2757  & 26.59 \\
		SwinIR~\cite{liang21swinir}
		& 11.90  & 708.61 & 5377 & 26.69 \\
		\midrule
		MetaSR~\cite{hu2019metasr}
		& 22.42 & 749.12 & 21381  & 25.99 \\
		LIIF~\cite{chen2021liif}
		& 22.32 & 810.75 & 10856 & 26.22 \\
		LTE~\cite{lee2021lte}
		& 22.47 & 781.59 & 8134  & 26.24 \\	
% 		\midrule
        \hline
		ITSRN~\cite{yang2021itsrn}
        & 22.62 & 888.67 & 20742 & 26.68 \\
		ITSRN++~
        & 13.98 & 502.10 & 12104 & 27.42 \\
        \hline

% 		\bottomrule[1.5pt]
	\end{tabular}
	}
\vspace{-2mm}
\end{table}
